LQ-LoRA: Low-rank Plus Quantized Matrix Decomposition for Efficient Language Model Finetuning

We propose a simple approach for memory-efficient adaptation of pretrained language models. Our approach uses an iterative algorithm to decompose each pretrained matrix into a high-precision low-rank component and a memory-efficient quantized component. During finetuning, the quantized component remains fixed and only the low-rank component is updated. We present an integer linear programming formulation of the quantization component which enables dynamic configuration of quantization parameters (e.g., bit-width, block size) for each matrix given an overall target memory budget. We further explore a data-aware version of the algorithm which uses an approximation of the Fisher information matrix to weight the reconstruction objective during matrix decomposition. Experiments on finetuning RoBERTa and LLaMA-2 (7B and 70B) demonstrate that our low-rank plus quantized matrix decomposition approach (LQ-LoRA) outperforms strong QLoRA and GPTQ-LoRA baselines and enables aggressive quantization to sub-3 bits with only minor performance degradations. When finetuned on a language modeling calibration dataset, LQ-LoRA can also be used for model compression; in this setting our 2.75-bit LLaMA-2-70B model (which has 2.85 bits on average when including the low-rank components and requires 27GB of GPU memory) performs respectably compared to the 16-bit baseline.

==> implementation.tex <==
\subsection{Implementation Details}
\label{subsec:implementation}
Here we discuss some  implementation details for efficiently implementing LQ-LoRA. We will make all our trained models and code publicly available upon publication.

\paragraph{PyTorch-based mixed-quantization.}
Weight-only quantization techniques typically require packing sub-8-bit matrices into natively-supported data types (e.g., \texttt{int8}), and then unpacking to float-point format during dequantization.  As such, existing implementations often require custom CUDA extensions that are dependent on a particular quantization configuration, making it difficult to extend to mixed-quantization strategies. Our implementation is based entirely on PyTorch for fast experimentation and implementation of dynamic quantization strategies. We use PyTorch’s \texttt{\_\_torch\_dispatch\_\_} functionality to duck-type \texttt{torch.Tensor},\footnote{\url{https://dev-discuss.pytorch.org/t/what-and-why-is-torch-dispatch/557}}  which redefines behaviors under PyTorch operations such as addition and matrix multiplication. We then use PyTorch’s (full-graph) compiler to compile the following operations: (1) bits-unpacking, (2) dequantization, (3) linear algebra operations such as \texttt{add} and \texttt{matmul}, and (4) transpose and casting (for \texttt{bf16} training). For LoRA finetuning, we observed this PyTorch-based implementation (followed by compilation) to be as fast as QLoRA's \texttt{bitsandbytes} implementation,\footnote{\url{https://github.com/TimDettmers/bitsandbytes}} which relies heavily on CUDA extensions that are tailored for  4-bit NF quantization.

\paragraph{LoRA optimizer offloading.}
We also work with  a CPU-based optimizer~\citep{ren2021zero}, which extends the pageable optimizer proposed in~\citet{dettmers2023qlora}. This implementation takes advantage of the fact that in LoRA, only a small portion of parameters needs to be trained, which makes data movement between CPU and GPU, as well as computation on CPU, relatively manageable. We retain a copy of trainable parameters on CPU, offload gradients from GPU to CPU before executing optimizer step on the parameter copy on CPU, and copy them back into GPU. We overlap the per-matrix optimizer step and CPU to GPU movement through async copy. On the largest 70 billion parameter model, we noticed a $14$\% memory saving with only a marginal (${<}2$\%) increase in training speed with this strategy.






==> rpca_algorithm.tex <==
\begin{minipage}{0.47\textwidth}
\centering
\begin{algorithm}[H]
\caption{LoST}\label{alg:rpca}
\begin{algorithmic}
\Require $\mathbf{A} \in \mathbb{R}^{n \times m}, T, r, b$
\State $\text{Initialize } \epsilon_0 \gets \infty$
\State $\text{Initialize } \mathbf{Q} \gets \mathbf{0}$
\For{$t \gets 1$ to $T$}
    \State {\color{gray}\text{\# factorization with randomized SVD}}
    \State $[\mathbf{U}, \mathbf{\Sigma}, \mathbf{V}^\top] \gets \operatorname{rSVD}(\mathbf{A} - \mathbf{Q}, r)$
    \State $\mathbf{L}_1 \gets \mathbf{U} \sqrt{\mathbf{\Sigma}}$
    \State $\mathbf{L}_2 \gets \sqrt{\mathbf{\Sigma}} \mathbf{V}^\top$
    \State {\color{gray}\text{\# quantization step}}
    \State $\mathbf{Q} \gets \operatorname{proj}_b\left(\mathbf{\mathbf{A} - \mathbf{L}_1 \mathbf{L}_2}\right)$
    \State {\color{gray}\text{\# stopping criterion}}
    \State $\epsilon_t \gets \|\mathbf{L}_1 \mathbf{L}_2 + \mathbf{Q} - \mathbf{A} \|_{F}$
    \If{$\epsilon_t > \epsilon_{t-1}$}
        \State break
    \EndIf
\EndFor
\Ensure  $\mathbf{L}_1, \mathbf{L}_2, \mathbf{Q}$
\end{algorithmic}
\end{algorithm}
\end{minipage}


